Credulous Users and Fake News: a Real Case Study on the Propagation in Twitter

Recent studies have confirmed a growing trend, especially among youngsters, of using Online Social Media as favourite information platform at the expense of traditional mass media. Indeed, they can easily reach a wide audience at a high speed; but exactly because of this they are the preferred medium for influencing public opinion via so-called fake news. Moreover, there is a general agreement that the main vehicle of fakes news are malicious software robots (bots) that automatically interact with human users. In previous work we have considered the problem of tagging human users in Online Social Networks as credulous users. Specifically, we have considered credulous those users with relatively high number of bot friends when compared to total number of their social friends. We consider this group of users worth of attention because they might have a higher exposure to malicious activities and they may contribute to the spreading of fake information by sharing dubious content. In this work, starting from a dataset of fake news, we investigate the behaviour and the degree of involvement of credulous users in fake news diffusion. The study aims to: (i) fight fake news by considering the content diffused by credulous users; (ii) highlight the relationship between credulous users and fake news spreading; (iii) target fake news detection by focusing on the analysis of specific accounts more exposed to malicious activities of bots. Our first results demonstrate a strong involvement of credulous users in fake news diffusion. This findings are calling for tools that, by performing data streaming on credulous' users actions, enables us to perform targeted fact-checking.

==> tabfeatures.tex <==
\begin{table*}[!htpb]
	\begin{center}
		\begin{tabular}{lcl}
			\hline
{\textbf{Name}} & \multicolumn{1}{c}{\textbf{Original Features}} & \multicolumn{1}{c}{\textbf{\makecell{Features alteration}}} \\ \hline
			\makecell[l]{\textbf{Botometer+}\\used in\cite{DBLP:conf/ideal/BalestrucciNPT19}\\ From Botometer\cite{Varol17}}& \makecell{Macro categories scores:\\
			Sentiment, Friend, \\
			User, Content, \\
			Temporal, Net } & \makecell[l]{ (+) CAP (ENG and UNI)\\
			(+) Score (ENG and UNI)\\
			(+) \#Tweets4WS %[ref SAC]
			\\
			(+) \#Mentions4WS %[ref SAC]
			}\\ \hline
			\makecell[l]{\textbf{ClassA-}\\used in\cite{DBLP:conf/ideal/BalestrucciNPT19}\\ From Fake Follower\cite{Cresci15fame}\\(Class A)}&  \makecell{friends/(followersˆ2), age, \\
			\#tweets, profile has name, \\
			has URL in profile, following rate, \\
			default image after 2 months, \\
			belongs to a list, profile has image, \\
			friends/followers$\geq$50, \\`bot' in biography, \#friends,\\
			2$\times$ followers $\geq$ friends, \\
			\#followers, friends/followers$\simeq$100, \\
			no bio \& no location \& friends$\geq$100, \\
			has address, has biography }& \makecell[l]{(-) duplicated pictures \\  of the profile }\\ \hline
		\end{tabular}
	\end{center}
	\caption{Feature sets}
	\label{tab:features}
\end{table*}
